OpenRSD: Towards Open-prompts for Object Detection in Remote Sensing Images

Remote sensing object detection has made significant progress, but most studies still focus on closed-set detection, limiting generalization across diverse datasets. Open-vocabulary object detection (OVD) provides a solution by leveraging multimodal associations between text prompts and visual features. However, existing OVD methods for remote sensing (RS) images are constrained by small-scale datasets and fail to address the unique challenges of remote sensing interpretation, include oriented object detection and the need for both high precision and real-time performance in diverse scenarios. To tackle these challenges, we propose OpenRSD, a universal open-prompt RS object detection framework. OpenRSD supports multimodal prompts and integrates multi-task detection heads to balance accuracy and real-time requirements. Additionally, we design a multi-stage training pipeline to enhance the generalization of model. Evaluated on seven public datasets, OpenRSD demonstrates superior performance in oriented and horizontal bounding box detection, with real-time inference capabilities suitable for large-scale RS image analysis. Compared to YOLO-World, OpenRSD exhibits an 8.7\% higher average precision and achieves an inference speed of 20.8 FPS. Codes and models will be released.

==> Tabels/Table10_Dataset_Sampling.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[b]
  \centering
  \caption{The datasets used in the pretraining and fine-tuning stages, along with their respective sampling rates.}
      \scriptsize
        \setlength{\tabcolsep}{10pt} % 将列间距设置为 3pt
    \begin{tabular}{c|c|c}
            \hline

    Name & Datasets & \multicolumn{1}{c}{Sampling Rates} \\
            \hline
    \multirow{3}[0]{*}{ORSD-Pre} & DOTA-v2.0, DIOR-R, FAIR1M-2.0 , & \multicolumn{1}{c}{8: 2: 8: } \\
        & SpaceNet, Xview, HRSC2016, & \multicolumn{1}{c}{2: 2: 1: } \\
        & GLH-Bridge, Million-AID & \multicolumn{1}{c}{4: 16} \\
        \hline
        
    \multirow{4}[0]{*}{ORSD+} & DOTA-v2.0, DIOR-R, FAIR1M-2.0, & \multicolumn{1}{c}{8: 2: 8:} \\
        & SpaceNet, Xview, HRSC2016,  & \multicolumn{1}{c}{2: 2: 0.5:} \\
        & GLH-Bridge, fMoW, WHU-Mix & 1: 4: 2:  \\
        & ShipRSImageNet & 0.5 \\
        \hline

    \end{tabular}%
  \label{tab:Table10_Dataset_Sampaling}%
\end{table}%

==> Tabels/Table10_Old.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[t]
  \centering
  \caption{The datasets used in the pretraining and fine-tuning stages, along with their respective sampling rates.}
      \scriptsize
        \setlength{\tabcolsep}{1.3pt} % 将列间距设置为 3pt
    \begin{tabular}{c|c|c}
            \hline

    Name & Datasets & \multicolumn{1}{c}{Sampling Ratios} \\
            \hline
    \multirow{3}[0]{*}{ORSD-Pre} & DOTA-v2.0 \cite{dota2}, DIOR-R \cite{diorr}, FAIR1M-2.0 \cite{sun2022fair1m}, & \multicolumn{1}{c}{8: 2: 8: } \\
        & SpaceNet \cite{spacenet}, Xview \cite{xview}, HRSC2016 \cite{hrsc2016}, & \multicolumn{1}{c}{2: 2: 1: } \\
        & GLH-Bridge \cite{li2024learning}, Million-AID \cite{maid} & \multicolumn{1}{c}{4: 16} \\
        \hline
        
    \multirow{4}[0]{*}{ORSD+} & DOTA-v2.0 \cite{dota2}, DIOR-R \cite{diorr}, FAIR1M-2.0 \cite{sun2022fair1m}, & \multicolumn{1}{c}{8: 2: 8:} \\
        & SpaceNet \cite{spacenet}, Xview \cite{xview}, HRSC2016 \cite{hrsc2016},  & \multicolumn{1}{c}{2: 2: 0.5:} \\
        & GLH-Bridge \cite{li2024learning}, fMoW \cite{christie2018functional}, WHU-Mix \cite{whumix} & 1: 4: 2:  \\
        & ShipRSImageNet \cite{zhang2021shiprsimagenet} & 0.5 \\
        \hline

    \end{tabular}%
  \label{tab:Table10_Dataset}%
\end{table}%

==> Tabels/Table11_STAR.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[t]
  \centering
  \caption{
  Open-set object detection performance on the STAR \cite{li2024star} dataset, including recall and precision for the categories 'Car,' 'Tool Gate,' and 'Cooling Tower,' as well as overall average recall (AR50) and AP50. Models marked with * are trained using the proposed ORSD+ dataset.}
      \scriptsize
       \setlength{\tabcolsep}{3.5pt} % 将列间距设置为 3pt
    \begin{tabular}{c|cc|cc|cc|cc}
    \hline
    \multirow{2}[2]{*}{Methods} & \multicolumn{2}{c|}{Car} & \multicolumn{2}{c|}{Tool Gate} & \multicolumn{2}{c|}{Cooling Tower} & \multirow{2}[2]{*}{AR50} & \multirow{2}[2]{*}{AP50} \\
        & Rec. & Pre. & Rec. & Pre. & Rec. & Pre. &     &  \\
    \hline
    CastDet* & 89.7  & 49.5  & 0.0  & 0.0  & 0.0  & 0.0  & 23.2  & 10.7  \\
    PKINet* & 82.7  & 48.1  & 0.0  & 0.0  & 2.9  & 0.0  & 25.9  & 10.8  \\
    OpenRSD (Text) & \textbf{98.2}  & \textbf{54.2}  & 47.4  & \textbf{6.8}  & 80.0  & 0.1  & 40.0  & 13.4  \\
    OpenRSD (Image) & 98.0  & \textbf{54.2}  & \textbf{68.4}  & 0.1  & \textbf{85.7}  & \textbf{66.5}  & \textbf{45.3}  & \textbf{13.5}  \\
    \hline
    \end{tabular}%

  \label{tab:Table11_Star}%
\end{table}%

==> Tabels/Table7_Restore.tex <==
\begin{table}[t]
  \centering
  \caption{Comparison of performance under different prompt types and quantities.}
    \footnotesize
      \setlength{\tabcolsep}{10pt} % 将列间距设置为 3pt
    \begin{tabular}{c|ccccc}
    \hline
        & 1   & 3   & 5   & 10  & 20 \\
    \hline
    \textit{\textbf{DIOR-R}} &     &     &     &     &  \\
    Image Prompt & 73.4  & 73.7  & 73.7  & 73.7  & 73.7  \\
    Text Prompt & 73.7  & 73.7  & 73.7  & 73.7  & 73.7  \\
    \hline
    \textit{\textbf{DOTA-v2.0}} &     &     &     &     &  \\
    Image Prompt & 65.7  & 67.8  & 67.8  & 68.2  & 68.0  \\
    Text Prompt & 70.1  & 70.2  & 70.1  & 70.1  & 70.1  \\
    \hline
    \textit{\textbf{HRSC2016}} &     &     &     &     &  \\
    Image Prompt & 87.9  & 87.7  & 88.1  & 88.1  & 88.0  \\
    Text Prompt & 88.1  & 88.3  & 88.6  & 88.0  & 87.7  \\
    \hline
    \textit{\textbf{FAIR1M-2.0}} &     &     &     &     &  \\
    Image Prompt & 44.0  & 44.0  & 44.1  & 44.1  & 44.0  \\
    Text Prompt & 46.0  & 45.9  & 46.1  & 46.1  & 46.0  \\
    \bottomrule
    \end{tabular}%
  \label{tab:Table7_Prompt}%
    \vspace{-3em}


\end{table}

==> Tabels/Table8_SamplingRatio.tex <==
\begin{table}[t]
  \centering
  \caption{Ablation study of dataset sampling rates.}
    \footnotesize
    \setlength{\tabcolsep}{3.2pt} % 将列间距设置为 3pt
    \begin{tabular}{c|cccc}
    \hline
    Sampling Rate & DIOR-R & DOTA-v1.0 & DOTA-v2.0 & FAIR1M-2.0 \\
    \hline
    Balance & 74.0  & 75.3  & 65.2  & 42.2  \\
    Emperical & 72.9  & 76.6  & 70.4  & 45.9  \\
    \hline
        & WHU-Mix & SpaceNet & HRSC2016 & Average \\
    \hline
    Balance & 79.9  & 50.7  & 89.2  & 68.1  \\
    Emperical & 79.4  & 47.5  & 84.6  & 68.2  \\
    \hline
    \end{tabular}%

  \label{tab:Table8_SamplingRatio}%
\end{table}
